Survey: Machine Learning in Production Rendering

In the past few years, machine learning-based approaches have had some great success for rendering animated feature films. This survey summarizes several of the most dramatic improvements in using deep neural networks over traditional rendering methods, such as better image quality and lower computational overhead. More specifically, this survey covers the fundamental principles of machine learning and its applications, such as denoising, path guiding, rendering participating media, and other notoriously difficult light transport situations. Some of these techniques have already been used in the latest released animations while others are still in the continuing development by researchers in both academia and movie studios. Although learning-based rendering methods still have some open issues, they have already demonstrated promising performance in multiple parts of the rendering pipeline, and people are continuously making new attempts.

==> experiments.tex <==


\section{Experiments}
We now present a comprehensive evaluation of our method.
%by comparing our network with other network variants and showing results on novel scenes with complex caustic effects

\paragraph{Ablation study.}
We first justify the choices of our network design.
In particular, 
we compare our network with a baseline network that estimates the final radiance without predicting kernels;
this comparison network has a similar network architecure but directly outputs the final irradiance from the across-photon deep context vector.
%We also compare against our network without using Eqn.~\ref{eqn:mapping} for normalization.
Figure~\ref{fig:opt} shows the training processes of these networks;
our network converges significantly faster than the baseline method.
This demonstrates the effectiveness of combining kernel density estimation and deep learning and is consistent with previous results on denoising for path tracing \cite{bako2017kernel,vogels2018denoising,gharbi2019sample}.


\begin{figure}[h]
    \includegraphics[width=\linewidth]{figs/loss.pdf}
    \caption{Optimization speed. We compare the optimization speed of our kernel-prediction network, and a baseline direct-estimation network.  Our network converges faster to the lower loss value.}
    \label{fig:opt}
\end{figure}

 



\paragraph{Evaluation scenes and settings.}
We evaluate our method on four challenging scenes (\Scenea, \Sceneb, {\Scenec}, \Scened)
that involve complex caustics and other diffuse-specular interactions with LS paths.
In theory, LS paths can never be reconstructed by path tracing if we use a point light source; we therefore use area lights in the scenes to allow for reasonable comparisons with PT.
For each scene, we shoot photons for 1 second and only keep those photons that involve light-specular paths.
We denote the number of valid photons we consider as $M$, which is a number that is different from the total emitted photon paths $N$ in Eqn.~\ref{eqn:kernel}.
Because of various compositions of scenes, there are 15k (\Scenea), 85k (\Sceneb), 54k (\Scenec), and 49k (\Scened) valid photons that are used in the four scenes respectively.
We also evaluate with the number of photons that are traced in ten seconds---corresponding to ten times the number of photons traced in one second---to justify the generalization of our network to different numbers of emitted photons.
We observe that it is very hard for a single network to generalize across different numbers of input photons ($\PhotonNN$).
We thus use a fixed $\PhotonNN$ when training per network, and specifically we train two networks with $\PhotonNN=50$ and $\PhotonNN=500$ for the evaluation.

\begin{figure}
    \includegraphics[width=\linewidth]{figs/pt.pdf}
    \caption{Path tracing and (PT) without light-specular paths (LS). We show PT and denoising results using 100 spp with and without light-specular paths.  The noise can be seen more clearly when 
    zooming into the electronic PDF.}
    \label{fig:pt}
\end{figure}


\begin{table*}[t]
	\begin{center}
		%\resizebox{\linewidth}{!}{
        \begin{tabular}{ | c c c | }  
        \multicolumn{3}{|c|}{\Scenea}\\
        \hline       
        ($\PhotonNN$,$M$)          & Ours  & PM \\
                    \hline
        (50, 15k)   & 0.00356 & 0.01902   \\
        \hline
        (50, 150k)  & \blue{0.00308} & \blue{0.00522}   \\
        \hline
        (500, 15k)  & \red{0.00380} & 0.04225   \\
        \hline
        (500, 150k) & 0.00308 & 0.01838   
        \end{tabular}
        \begin{tabular}{ | c c c | }
        \multicolumn{3}{|c|}{{\Sceneb}}\\
        \hline 
        ($\PhotonNN$,$M$) & Ours  & PM \\
                    \hline
        (50, 85k)   & 0.03497 & 0.06870   \\
        \hline
        (50, 850k)  & 0.02570 & \blue{0.03221}   \\
        \hline
        (500, 85k)  & \red{0.03513} & 0.1311   \\
        \hline
        (500, 850k) & \blue{0.02038} & 0.06012   
        \end{tabular}
        \begin{tabular}{ | c c c | }
        \multicolumn{3}{|c|}{{\Scenec}}\\
        \hline 
        ($\PhotonNN$,$M$)   & Ours  & PM \\
            \hline
        (50, 54k)   & 0.01934 & 0.03441   \\
        \hline
        (50, 540k)  & \red{0.02084} & \blue{0.02098}   \\
        \hline
        (500, 54k)  & 0.01539 & 0.0915   \\
        \hline
        (500, 540k) & \blue{0.00875} & 0.02365   
        \end{tabular}
        \begin{tabular}{ | c c c | }
        \multicolumn{3}{|c|}{{\Scened}}\\
        \hline 
        ($\PhotonNN$,$M$)  & Ours  & PM \\
            \hline
        (50, 49k)   & \red{0.2320} & 0.2607   \\
        \hline
        (50, 490k)  & 0.2001 & \blue{0.2032}   \\
        \hline
        (500, 49k)  & 0.2164 & 0.3057   \\
        \hline
        (500, 490k) & \blue{0.1410} & 0.2237   
        \end{tabular}
		%}
        \caption{Quantitative RMSE evaluation. We test our two networks ($\PhotonNN=50$ and $\PhotonNN=500$) on four novel  scenes with different numbers of emitted photons,
         and compare RMSE against standard photon mapping \cite{jensen1996global} under the same conditions. Photon mapping's performance varies widely based on the settings but the best results (shown in \blue{blue}) are always with high photon count and $K=50$ nearest neighbors. On the other hand, our results are more consistent with different settings, demonstrating our networks' ability to adapt to different numbers of traced photons. Moreover, our worst results (shown in \red{red}) are usually with low photon counts and are similar to, if not better than the best photon mapping results (with 10x more photons). Meanwhile, our best results (shown in \blue{blue}) are at higher photon counts and have substantially lower errors than photon mapping with the same photon counts.}
		\label{tab:rmses}
	\end{center}
\end{table*}

\begin{figure*}
    \includegraphics[width=\linewidth]{figs/results_NK.pdf}
    \caption{Visual demonstration for Tab.~\ref{tab:rmses}. We show results of our method with different numbers of input photons ($\PhotonNN$) and total photons ($M$).  We compare against photon mapping with the same settings on insets marked in the left-most ground truth image. The PSNRs and SSIMs of the insets are also shown correspondingly.}
    \label{fig:resultsNK}
\end{figure*}


\paragraph{Combining MC denoising and deep photon mapping.}
We evaluate our deep photon density estimation by combining our method with MC denoising. 
Specifically, we apply our learning-based density estimation to only compute the challenging light transport effects
which involve LS paths that are extremely hard to trace in PT and likely to introduce caustics.
In addition, we use path tracing with relatively low sample counts to compute the remaining light transport paths, 
and use modern learning-based denoising---the Optix built-in denoiser based on \cite{chaitanya2017interactive}---to remove the MC noise.

By removing LS paths in PT, we also make PT and MC denoising much easier. 
As shown in Fig.~\ref{fig:pt}, 
PT without LS paths can be effectively denoised using modern learning-based denoising techniques with 100 spp, whereas full PT with LS paths introduces extensive noise with the same 100 spp, causing denoising to fail completely.
In fact, the standard PT plus denoising pipeline is not able to recover the complex light transport effects with even 1000 spp (see Figs.~\ref{fig:teaser},\ref{fig:results}).
In contrast, we demonstrate a practical way of combining our efficient deep photon mapping with MC denoising for photorealistic image synthesis, in which we leverage the benefits of low-sample reconstruction in both scene-space particle density estimation and screen-space MC integration.

\begin{figure*}[t]
    \includegraphics[width=\linewidth]{figs/results.pdf}
    \caption{We show our results on full images (a), and compare against photon mapping (c) and pure path tracing (e) with 1000 spp with insets. The images purely generated from our method and photon mapping for LS paths are shown in (g), (h) respectively. We combine these images with PT denoising using 300 spp for \Scenea~and 100 spp for the other three scenes. PSNRs and SSIMs are also calculated for all insets and listed below.}
    \label{fig:results}
\end{figure*}


%Note that, since our networks always deal with photons normalized in a unit sphere as input, each network is well generalized across different radii with different number of total photons.

%\paragraph{Combining MC denoising and deep photon mapping.}
%Path tracing (PT) with MC denoising has been widely used in fast rendering with global illumination;
%however, complex effects with light-specular (LS) paths, like caustics are very difficult for this denoising solution to simulate, 
%which typically requires the involvement of photon mapping for efficient computation.

\paragraph{Evaluation on different input settings.}
We now evaluate our method quantitatively and qualitatively with different numbers of input
photons ($\PhotonNN$) and different numbers of valid photons in a scene ($M$).
Table ~\ref{tab:rmses} shows quantitative RMSE evaluation of photon density estimation on the four testing scenes; the numbers are averaged across about 260k surface shading points sampled by tracing rays from a camera and selecting the first diffuse hit points in the scenes.
Note that, in all these different input settings, 
our method is consistently better than standard photon mapping \cite{jensen1996global}.
In fact, most of our results are better than photon mapping with ten times the photon counts as ours.
Besides, photon mapping is very sensitive to different settings. This is shown by noting that the RMSEs of photon mapping vary significantly, whereas our method is very stable across different settings.

Across these four scenes, photon mapping clearly favors a greater number of photons and fewer nearest neighbor photons (corresponding to a smaller bandwidth); in Tab.~\ref{tab:rmses}, this setting is always the best for photon mapping.
For a standard kernel, this setting focuses more on good caustic effects that have high densities of photons. 
However, it is very hard to avoid non-smooth artifacts in regions with sparse photons.
We demonstrate the rendering results of \Scenec~and~\Scened~with all four input settings in Fig.~\ref{fig:resultsNK} to visually illustrate the numbers in Tab.~\ref{tab:rmses}.
Note that, photon mapping either introduces obvious non-smooth artifacts with a small bandwidth (Fig.~\ref{fig:resultsNK}.i and Fig.~\ref{fig:resultsNK}.g) or outputs over-smooth results without details with a large bandwidth (Fig.~\ref{fig:resultsNK}.c and Fig.~\ref{fig:resultsNK}.e).
In contrast, our method is able to leverage more photons in a large bandwidth without introducing any obvious over-smoothing issues.
This is thanks to our learning based context-aware kernel prediction approach.
In particular, our approach allows for every single photon to leverage across-photon information in the learned deep context feature to tell if it is an outlier or an important contributing element to the shading point's reflected radiance; a corresponding kernel weight is assigned to each photon based on the decision made by data priors in the network.
Therefore, our method is able to effectively utilize the sparse photons in a large area to generate photorealistic images that are of high smoothness and have many details.

\paragraph{Additional results on testing scenes.}
We show more results of the four test scenes in Fig.~\ref{fig:results}, where we compare with photon mapping and path tracing results. We also show the images generated from our network before being combined with low-sample path tracing and denoising.
Our results are significantly better than the photon mapping results and are closer to the ground truth, which is reflected by better visual quality and higher quantitative numbers in both the pure PM-based results (Fig.~\ref{fig:results}.g, h, i) and the final results (Fig.~\ref{fig:results}.b, c, d).
Moreover, path tracing (PT) plus denosing alone is clearly not able to handle the complex specular-diffuse interactions in these scenes; the PT with denoising results (Fig.~\ref{fig:results}.e) either introduces obvious artifacts or misses the caustics.
Note that, PT plus denoising results with 1000 spp are still significantly worse than ours that are using almost an order of magnitude fewer path (100 spp or 300 spp) and photon (less than 4 photons per pixel) samples.
We demonstrate the benefits of combining our deep photon mapping and MC denoising, which enables efficient photorealistic rendering with complex global illumination.

\paragraph{Timing.}
We use Optix to trace photons and do path tracing for all the results.
All experiments are run on one NVIDIA 1080 Ti GPU.
It takes about 1 second to generate 15k, 85k, 54k and 49k valid photons for \Scenea, \Sceneb, \Scenec, \Scened~respectively.
Our KNN searching is done on the CPU, which takes about 1 to 3 seconds to find neighbors for 260k shading points. 
Path tracing runs at about 50 spp per second in all four scenes with an image resolution of 512$\times 512$.
Note that the running time of our network is linear with the number of input photons $\PhotonNN$, and it is also determined by the number of shading points that are required to be computed.
In particular, it takes about $0.2$s with $\PhotonNN=50$ and $2$s with $\PhotonNN=500$ for our network to compute about 260k shading points, corresponding to 1 point per pixel in a $512 \times 512$ image.

\paragraph{Temporal consistency.}
Since our method deals with shading points in 3D space and is independent of view directions, we have observed that it has good across-frame consistency when changing the view in a scene with a fixed set of photons. 
We leave the extensions of general temporal consistency with other dynamic components in a scene as future work.

\paragraph{Progressive density estimation.}
Our current framework requires a fixed number of input photons for each trained network.  Progressive photon mapping accepts different numbers of photons per iteration with reduced bandwidth. 
Nonetheless, we have demonstrated that our network architecture supports accurate photon density estimation
with various fixed photon numbers. 
In other words, a progressive method can potentially be achieved by training a sequence of networks with different numbers of inputs.
A universal network for any given number of input photons may require introducing recurrent networks in the framework, which is an interesting direction of future work. 

%\paragraph{Network settings.}
%Note that, since our network deals with individual photons, the running time is linear with $\PhotonNN$. 
%In particular, it takes about $0.2$s with $\PhotonNN=50$ and $2$s with $\PhotonNN=500$ for our network to compute a $512 \times 512$ image on an NVIDIA 1080TI GPU. 

%\paragraph{Network settings.}
%Note that, since our network deals with individual photons, the running time is linear with $\PhotonNN$. 
%In particular, it takes about $0.2$s with $\PhotonNN=50$ and $2$s with $\PhotonNN=500$ for our network to compute a $512 \times 512$ image on an NVIDIA 1080TI GPU. 

%where every photon can its kernel weight and tell if it is an outlier for the shading point by leveraging across-photon information in the deep context feature. 

%which is not a very bad choice for a scene whose LS paths are mostly focused on small regions with thin-structure caustics like   

%We also demonstrate the corresponding renderings of the the scene \Scenea and \Scenec with the different input settings in Fig.~\ref{fig:resultsNK}.














\section{Conclusions and Future Work}
In this paper, we have presented the first deep learning-based method for density estimation in particle-based rendering. We introduce a deep neural network that learns a kernel function to aggregate photons at each shading point and renders accurate caustics with significantly fewer photons than previous approaches, with minimal overhead. Learning-based MC denoising has significantly improved path tracing results and our work extends these benefits to the popular photon mapping method.  

%In the future, we would like to connect the particle-based denoising approach for photon mapping with the more image-space approaches in use for path tracing; we have already shown examples in our results of combining the techniques. % essentially in terms of separate passes. 
Our method could be improved in the future with more advanced machine learning approaches, perhaps based on generative adversarial networks (GANs), just as has been done with path tracing \cite{xu2019adversarial}.  More broadly, we believe this paper points towards denoisers specialized to many other approaches for realistic image synthesis such as Metropolis Light Transport and Vertex Connection and Merging.   
